Proportional-Integral Projected Gradient Method for Conic Optimization

Conic optimization is the minimization of a differentiable convex objective function subject to conic constraints. We propose a novel primal-dual first-order method for conic optimization, named proportional-integral projected gradient method (PIPG). PIPG ensures that both the primal-dual gap and the constraint violation converge to zero at the rate of \(O(1/k)\), where \(k\) is the number of iterations. If the objective function is strongly convex, PIPG improves the convergence rate of the primal-dual gap to \(O(1/k^2)\). Further, unlike any existing first-order methods, PIPG also improves the convergence rate of the constraint violation to \(O(1/k^3)\). We demonstrate the application of PIPG in constrained optimal control problems.

==> experiment/muffin.tex <==
\begin{tikzpicture}[scale=0.4]
\draw[color=blue, fill=blue!15] (135:2.82) --  (135:5) arc (135:45:5) -- (45:2.82) -- cycle;

\draw[-, color=blue] (135:5) -- (45:5);

\draw[dashed] (135:2.82) -- (0,0) (45:2.82) -- (0, 0) (0, 0) --(2, 0);

\draw[-] (2, 2) --(2.8, 2) (2, 0)--(2.8, 0);
\draw[latex-latex] (2.4, 2) -- (2.4, 0) node[midway,right]{\footnotesize $\rho_{\min}$};


\draw[latex-latex]  (135:0.8) arc(135:45:0.8) node[midway,above]{\footnotesize $2\theta$};
\draw[rotate around={45:(0,0)}] (-0.8, 5) -- (0, 5) (-0.8, 0) -- (0, 0);
\draw[latex-latex, rotate around={45:(0,0)}] (-0.4, 5) -- (-0.4, 0) node[midway,left]{\footnotesize $\rho_{\max}$};

%\node at (0, 0)[circle,fill,inner sep=1pt]{};

\end{tikzpicture}

==> preliminary/triangle.tex <==
\begin{tikzpicture}[scale=0.7]
\coordinate (A) at (0,0);
\coordinate (B) at (2,0);
\coordinate (C) at (1,1.5);

\draw (0.3, 0) arc (0:56:0.3cm);

\node at (0.5, 0.3) {$\theta$};

\draw (A) -- (B) node[midway,below] {$a$}
   -- (C) node[midway,right] {$c$}
   -- (A) node[midway,left] {$b$};

\node at (7, 0.75) {\(-2ab\cos\theta=c^2-a^2-b^2\)};

\end{tikzpicture}
